Biocompatible Vaterite Carriers Enable Multimodal Quantum Sensing with Nanodiamonds

Mobile nanodiamond quantum sensors in liquids are affected by Brownian rotation, variable photon collection, and perturbations from optical trapping. Here we assemble 40-nm nitrogen-vacancy nanodiamonds on porous, birefringent vaterite microspherulites, creating mobile sensors with a polarization-addressable body frame and a chemically active carbonate interface. Under 976-nm trapping, the sensors retain spin resonance and longitudinal relaxation, with less than 7% variation in contrast and an approximately 1-MHz resonance shift at 0.8 W. Zeeman-split resonances resolve magnetic fields from 0 to 0.8 mT, with a response metric of 78--144 $\mu$T Hz$^{-1/2}$. In cell-culture medium, a 10.7-$\mu$M proton-equivalent dose shortens $T_1$ from $23.4 \pm 2.3$ to $9.0 \pm 1.2$ $\mu$s, yielding concentration and pH sensitivities of $6.46$ $\mu$M Hz$^{-1/2}$ and $6.54$ mpH Hz$^{-1/2}$, respectively. A 500-fold larger proton dose in ethanol produces a weaker response. A grand-canonical charge-regulation model links proton chemical potential to interfacial switching, establishing a route to multimodal quantum sensing in complex liquids.

==> Appendices.tex <==
%\section {\Large\textbf{Appendix A: Cathodoluminescence Characterization of Vaterite}}

Figure~\ref{fig:A1} shows the cathodoluminescence (CL) spectrum of vaterite particles collected under 30~keV electron-beam excitation. The spectrum exhibits a prominent emission peak at approximately 405~nm, corresponding to the intrinsic luminescence of the vaterite crystal lattice. This measurement supports the statement in the main text, confirming that the observed peak originates from the vaterite host itself.
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{Figures/figA1.png}
\caption{Cathodoluminescence characterization of vaterite. (a) CL maps were acquired using a 30~keV electron beam at 17~nA. (b) CL spectrum of vaterite, showing a prominent peak at 405~nm corresponding to the intrinsic luminescence of the vaterite host.}
    \label{fig:A1}
\end{figure}

==> Optomechanical_locking_and_photonic_gain.tex <==
The vaterite carrier is a passive birefringent scaffold with an additional photonic role. In a linearly polarized optical trap, its optical anisotropy produces a restoring torque that stabilizes a body-fixed axis in liquid. The same anisotropy can redistribute emission from surface-bound nanodiamonds into an orientation-dependent angular pattern. To quantify this effect, we performed FDTD simulations for dipole emitters located at the particle surface in solution and analyzed the resulting near fields and far-field radiation patterns (see Appendix B).

For surface-bound nanodiamonds, dipoles aligned with the vaterite optical axis give rise to a pronounced forward-directed emission lobe, consistent with photonic nanojet formation along the extraordinary axis of the birefringent vaterite sphere. In the near field, this configuration supports efficient funneling of electromagnetic energy at the particle surface (Fig.~\ref{fig:fig4}a), while the corresponding far-field response exhibits a strongly collimated emission channel directed along the optical axis (Fig.~\ref{fig:fig4}b). Dipole orientations and positions away from this configuration result in comparatively isotropic and less efficient radiation patterns, with the full set of near- and far-field cases provided in the Appendix~\cite{ref16}. The anisotropic refractive tensor of vaterite acts as a mesoscopic birefringent lens and can support non-Mie resonances and directional scattering in related biomineral structures~\cite{ref15,ref16,ref18}. The resulting modification of the local photonic environment is captured by the Purcell factor (Fig.~\ref{fig:fig4}c), which exhibits a modest but non-negligible enhancement averaged over dipole orientations, with additional averaging over different positions within the hybrid particle provided in the Appendix. This enhancement remains consistent across the NV emission band.

The key implication of these calculations is that vaterite acts as an intrinsic directional optical element, redistributing emission into a structured angular pattern while remaining transparent in the visible, thereby enhancing collection efficiency without the need for nanofabricated photonic structures. Additional simulations examining the electric field distribution and Purcell factor for different dipole positions within the vaterite particle, as well as the effects of particle diameter and nanodiamond size, are provided in Appendix B.

Experimentally, single hybrids were trapped in heavy water (D$_2$O) with a linearly polarized 975--976 nm beam. Rotating a quarter-wave plate rotated the trapping polarization and therefore the orientation of the birefringent particle. The detected PL varied periodically with rotation angle, with two maxima separated by 180$^\circ$ (Fig.~\ref{fig:4}d), consistent with an orientation-dependent emission pattern and collection efficiency. This result shows that, unlike freely diffusing nanodiamonds, the hybrid microcarrier maintains a stable photoluminescence and addressable orientation in liquid (see Appendix B2).

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=3mm,right=3mm,top=10mm,columnsep=10pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{float}
\usepackage{wrapfig}
\captionsetup{subrefformat=parens}

% \usepackage{subfigure}
